The single-use restriction for register automata and transducers over infinite alphabets

This thesis studies the single-use restriction for register automata and transducers over infinite alphabets. The restriction requires that a read-access to a register should have the side effect of destroying its contents. This constraint results in robust classes of languages and transductions. For automata models, we show that one-way register automata, two-way register automata, and orbit-finite monoids have the same expressive power. For transducer models, we show that single-use Mealy machines and single-use two-way transducers admit versions of the Krohn-Rhodes decomposition theorem. Moreover, single-use Mealy machines are equivalent to an algebraic model called local algebraic semigroup transductions. Additionally, we show that single-use two-way transducers are equivalent to single-use streaming string transducers (SSTs) over infinite alphabets and to regular list functions with atoms. Compared with the previous work arXiv:1907.10504, this thesis offers a coherent narrative on the single-use restriction. We introduce an abstract notion of single-use functions and use them to define all the discussed single-use models. We also introduce and study the algebraic models of local semigroup transduction and local rational semigroup transduction.

==> register-automata-2.tex <==
\chapter{Register automata and sets with atoms}\label{sec:register-automata}

Let us consider an infinite set of atoms ($\atoms$). Informally, the elements
of this sets can only be compared for equality (formal definition appears
later in this chapter). This idea is quite similar to
abstract data types(ADTs) known from many programming languages --
$\atoms$ could be expressed as an abstract set whose interface
only contains equality predicate. For example in Haskell, set $\atoms$
could be expressed as:
\[\mathtt{Eq\ a \ \Rightarrow a}\footnote{Keeping in mind that $\atoms$ has to be infinite}\]

One can extend classical automata to work with languages over $\atoms$.
In order to deal with
the infinite alphabets they are equipped with a finite set of registers
for storing elements of $\atoms$ (in addition to the finite set of states).
Before providing a formal definition we give a couple of examples.
\begin{example}
    The language ``The first letter appears again'' can be recognised by
    a register automaton with one register and three states: the automaton remembers
    the first letter in the register and compares every other letter to the register
    value.
    \picc{first-again}
\end{example}
\begin{example}
    The language ``There are at most $3$ different letters can be recognized''
    by a register automaton with $2$ states and $3$ registers: the automaton
    saves each new letter in a register. It rejects after it sees the fourth letter.
    \picc{at-most-3}
\end{example}

We see now that a deterministic register automaton consists of a finite set of states $Q$,
and a finite number of registers $k$. Its transition function is of the type:
\[\underbrace{Q \times (\atoms + \bot)^k}_{\substack{\textrm{current state} \\  \textrm{and register valuation}}}
\times \underbrace{\atoms}_{\textrm{new letter}} \to
\underbrace{Q \times (\atoms + \bot)^k}_{\substack{\textrm{new state} \\  \textrm{and register valuation}}}\]
We cannot, however, allow for arbitrary function of this type. If we did, already a one-registers automata could
easily simulate arbitrary infinite-state machines, which can recognize all the languages.
To limit the power of the automata, we formalize the restriction that elements of $\atoms$ should
only be compared for equality. There are $3$ equivalent ways of doing that.

The first one, called \emph{syntactic equivariance} \cite[p. 6]{bojanczyk_book}, requires the transition
function (treated as a relation) has to be a boolean combination of the following conditions:
\begin{itemize}
    \item the current/new state is equal to $q \in Q$
    \item register $i$ is empty in the current/new register valuation
    \item the input letter is equal to the value of register $i$ from the
          current/new situation
    \item the value of register $i$ from the current/new register valuation
          is equal to the value $j$ from the current/new register valuation
\end{itemize}

Another way, called \emph{semantic equivariance} \cite[p. 6]{bojanczyk_book}, states
that the function should be invariant under atoms renaming. In order to
formalize it, we notice that every atom permutation $\pi : \atoms \to \atoms$
can be extended to larger sets built from atoms; in particular to
$(Q \times (\atoms + \bot)^k)$ and to $(Q \times (\atoms + \bot)^k) \times \atoms$.
A transition function is syntactically equivariant, if it commutes with those actions
i.e. for all $x$ and $\pi$, it satisfies the following equation:
\[f(\pi(x)) = \pi(f(x)) \]

Finally, invoking the similarities with abstract data types, we can require
the transition function to be implementable in Haskell as a function of the type
\[\mathtt{Eq\ a \ \Rightarrow \ (Q,\ (Maybe\ a)^k, a) \to (Q, (Maybe\ a)^k) } \]
where $\mathtt{x^k}$ is a macro for the $k$-tuple $\mathtt{(x, x, \ldots, x)}$.

\begin{lemma}
    All three notions of equivariance are equivalent.
\end{lemma}
\begin{proof}
    Semantic and syntactic equivariance are equivalent thanks to \cite[Lemma~1.3]{bojanczyk_book}.
    The fact that every Haskell function of the correct type is semantically equivariant comes
    (for free) from \cite[Section~3.4]{wadler1989theorems}. The last fact to prove is that
    every syntactically equivariant function can be expressed as a Haskell function (of the correct type).
    The boolean combination of atomic condition can be expressed in a disjunctive normal form
    \[ \underbrace{(A \cap \neg B \cap C)}_{\textrm{clause 1}} \  \cup \ 
       \underbrace{(D \cap E)}_{\textrm{clause 2}} \ \cup \ \ldots \ \cup \
       \underbrace{(X \cap Y \cap \neg Z)}_{\textrm{clause } n} \]
    where each letter represents an atomic condition. We can use this representation to
    compute the transition function in Haskell:  First, compute the
    logical value of each atomic expression referring to the input configuration or to the input letter.
    Find a clause that satisfies all those properties, and based on the clause compute the output --
    it has to be uniquely defined because the boolean combination describes a function.
\end{proof}



\section{Sets with atoms}
Notice that the only interface needed to define equivariance was applying permutation of atoms, to an
element. We use this observation to extend the notion of equivariant functions to a broader class of sets.
This is based on based on \cite[Setcion 1.1~and Section~2.1]{pitts2013nominal} and \cite[Section 2]{bojanczyk2013nominal}.

We want to consider sets that can be transformed by permutations of the atoms. In order to formalize this intuition,
we use the definition of a group action on a set.

\begin{definition} \label{def:group-action} 
    A (left-)action of a group $G$ on a set $X$ is a function:
    \[ G \times X \to X \]
    (denoted as as $gx$, for $g \in G$ and $x \in X$). The action has to be compatible with the structure
    of the group, as asserted by the following axioms:
    \begin{itemize}
        \item $1 x = x$, for all $x \in X$
        \item $(gh)x = g (hx)$, for all $g, h \in G$, $x \in X$ (note the overloaded notation for
        group multiplication and group action).
    \end{itemize} 
\end{definition}

Our focus are sets equipped with an action of the group of all atom permutations(automorphisms)\footnote{Further in the paper we will also consider automorphisms that consider some more structure}
\[\auts \  \subseteq \  \atoms \to \atoms \]
It is useful to limit our considerations to elements can can be described using a finite number of atoms.
This can be formalized in the group-action setting, using the notion of \emph{supports}:

\begin{definition} \label{def:support} 
    Take a set $X$, equipped with the action of atoms automorphisms. We say that an element $x \in X$
    \emph{is supported by} a subset of atoms $A \subseteq \atoms$, if every atom automorphism that preserves
    every element of $A$ also preserves $x$:
    \[ \displaystyle\mathop{\forall}_{\pi \in \auts} \ \left(\displaystyle\mathop{\forall}_{a \in A}\pi(\bar a) = \bar a)\right) \ \Rightarrow \ \pi x = x   \]
    (Call such $A$-preserving automorphism an $A$-automorphism.)
\end{definition}

Now we are ready to define \emph{sets with atoms}:

\begin{definition} \label{def:sets-with-atoms}
    A \emph{set with atoms} is a set equipped with an action of atom automorphisms,
    such that every element has a finite support.
\end{definition}

It is worth noting that every element of a sets with atoms element has infinitely many supports
(if $A \subseteq B$ and $A$ is a support then $B$ is also a support), but it always has a minimal one
(with respect to set inclusion). This has been proven as \cite[Proposition~3.10]{gabbay2002new}:

\begin{theorem}\label{thm:least-support}
    If $x$ is an element of a set with atoms, then there is a unique $\supp(x) \subseteq \atoms$, which satisfies both of
    the following conditions:
    \begin{enumerate}
        \item $\supp(x)$ supports $x$
        \item $\supp(x)$ is contained in every support of $x$
    \end{enumerate}
    We say that en element $x$ is \emph{equivariant}, if $\supp(x) = \emptyset$.
\end{theorem}

Let us consider some examples of sets with atoms:

\begin{example}
    The set of all atoms $\atoms$, with the natural action $\pi x = \pi(x)$ is a set with atoms --
    each $a \in \atoms$ is supported by $\{a\}$.
\end{example}

\begin{example}
    The singleton set $1 = \{ \circ \}$, with the trivial action $\pi \,\circ = \circ$ is a set
    with atoms -- the element $\circ$ is supported by the empty set.
\end{example}

\begin{example}
    If $A$ and $B$ are sets with atoms, then their product $A \times B$, equipped with the natural action
    \[\pi \langle a, b \rangle = \langle \pi a, \pi b \rangle \]
    is a set with atoms -- $\supp(\langle a, b \rangle) = \supp(a) \cup \supp(b)$.
\end{example}

\begin{example}
  If $A$ and $B$ are sets with atoms, then their disjoint sum equipped with the natural action
  \[\pi \mathtt{left}(a) = \mathtt{left}(\pi a) \ \ \ \pi \mathtt{right}(b) = \mathtt{right}(\pi b)\]
  is also a set with atoms -- $\supp(\mathtt{left}(a)) = \supp(a)$ and $\supp(\mathtt{right}(a)) = \supp(a)$.
\end{example}

\begin{example}
    If $A$ is a set with atoms, then the set $A^*$ equipped with the natural action
    \[\pi (a_1 a_2 \ldots a_k) = \pi a_1 \pi a_2 \ldots \pi a_k\]
    is also a set with atoms -- $\supp(a) = \bigcup \supp(a_i)$
\end{example}

\subsection{Orbit-finiteness}
One can easily see that finiteness is neither useful nor interesting in the realm of sets with atoms --
virtually all interesting examples of sets with atoms are infinite. We can however relax the notion to
\emph{orbit-finiteness}, which means finite up to atom permutations: Define an orbit of an element:
\[\orbit(x) = \{\pi x \ | \ x \in \auts\}\]


\begin{claim}
    If a set with atoms $X$, contains an element $x$, such that $\supp(x) \neq \emptyset$,
    then $X$ is infinite.
\end{claim}
\begin{proof}
    Take such an $x$, then there exists $\pi$ such that $\pi x \neq x$. 
\end{proof}
\noindent
but, the set $\atoms^*$ seems \emph{more infinite} then the set $\atoms^2$. This intuition can
be formalized as \emph{orbit-finiteness}.









==> register-automata.tex <==
\chapter{Register automata and sets with atoms}\label{sec:register-automata}

This section serves to provide some context. For the most part of it, we consider an infinite alphabet
whose elements can only be compared for equality. We open the section with a concrete and low-level definition
of {\em deterministic register automaton}. To make it compatible with the single-use restriction
(defined in the subsequent chapters),
we give a definition that slightly differs from original one in~\cite[Defnition~1]{kaminski_finite_memory_paper}.
Both definitions follow, however, the same lines are easily seen to be equivalent. Next, we go to~\cite[Chapter~3]
{bojanczyk_book} and introduce {\em orbit-finite sets with atoms}. Then, following the narration of~\cite[Section~5.2]{bojanczyk_book}, we provide an abstract, high-level definition of a language acceptor equivalent
to the deterministic register automaton -- {\em deterministic orbit-finite automaton}.
Finally, we go beyond equality atoms and discuss atoms with more complex signatures, 
like total-order atoms. Keeping to~\cite[Section~5.2]{bojanczyk_book}, we give a sufficient condition on the atoms,
for which deterministic register automaton and deterministic orbit-finite automata are equivalent.

\section{Register automata}
\todo[inline]{Add an introduction about intuitions (programming language) and some examples}

\begin{definition}
    A syntax of a \emph{register automaton} consists of:
    \begin{enumerate}
        \item A finite set $Q$ of \emph{control states};
        \item An \emph{initial state} $q_0 \in Q$;
        \item A finite set $R$ of \emph{registers};
        \item A transition function which maps each control state $q \in Q$ to
        \[ \underbrace {questions}_{\textrm{what question to ask}}
         \times \underbrace{
                (Q \times actions)}_{
                    \substack{
                        \textrm{what to do if the question} \\
                        \textrm{has a ``yes'' answer}
                    }
                    }\times \underbrace{(Q \times actions)}_{\substack{
                        \textrm{what to do if the question} \\
                        \textrm{has a ``no'' answer}
                    }}\]
        with the following finite set of questions:
        \begin{enumerate}
             \item\label{q:cmp1} is the current letter equal to the value of register~$r \in R$?
             \item\label{q:cmp2} are the values of registers $r_1, r_2 \in R$ equal?
             \item has the automaton reached the end of word?
        \end{enumerate}
        and the following finite set of actions:
        \begin{enumerate}
            \item store the current letter in the register $r \in R$
            \item go forward
            \item accept / reject
            \item clear\footnote{ Adding this action does not add anything to the expressive power of the model; we include it because it will simplify the reasoning in the upcoming sections.}
                 the contents of every register from $C \subseteq R$
        \end{enumerate}
    \end{enumerate}
\end{definition}
As previously mentioned this kind of an automaton serves as an acceptor of languages over $\atoms$. Its semantics is
straight-forward: A \emph{state} of the automaton is an element of the set:
\[\underbrace{Q}_{\textrm{control state}} 
    \times \underbrace{{(\atoms + \bot)}^R}_{
    \substack{
        \textrm{contents of the registers}\\
        \textrm{(some of which may be empty)}
    }}\]
A \emph{configuration} of the computation is an element of the set:
\[ \underbrace{(Q \times {(\atoms + \bot)}^R)}_{
        \textrm{current full state}
  }
   \times \underbrace{\atoms^*}_{\substack{
   \textrm{the sufix of the input}\\
   \textrm{that remains to be processed}
   }}
\]
The initial configuration of the computation consists of the initial control state,
the empty register valuation and the entire word reminding to be processed.
In order to obtain a run of the automaton, we start in the initial configuration
and keep applying the transition function (naturally extended to work on configurations)
until the automaton accepts or rejects. If the automaton causes an undefined behaviour, by
\begin{enumerate}
\item accessing the value of an empty registers, 
\item exiting the word from the right,
\item starting to loop, or
\item asking for the current letter when already at the end of the input,
\end{enumerate}
it immediately stops the run and rejects the input word. However,
thanks to the following Lemma, we do not have to worry about such cases.
\begin{lemma}\label{lem:one-way-can-never-fail}
    Every register automaton can be modified so that, it never causes undefined behaviour.
\end{lemma}
Most cases of undefined behaviour can be easily prevented by keeping appropriate (finite)
information in the control state. The most interesting case of looping is handled by the
following Lemma.
\begin{lemma}\label{lem:register-bounded}
    For each non-looping automaton, there is a number $k$, such that
    the automaton never stays in one position for more than $k$ steps.
\end{lemma}
\begin{proof}
    We will show that as long as the automaton stays put,
    there is only finitely many configurations it can reach: The automaton can be in one of $|Q|$ control states,
    and use at most
    \[ \underbrace{|R|}_{
            \substack{\textrm{the atoms that were present} \\
                      \textrm{in the registers when} \\
                      \textrm{the automaton first entered the position}}} +
       \underbrace{1}_{\substack{
                        \textrm{the input atom}\\
                        \textrm{from the current position}}} \]
    different atoms. The automatons does not move, which by definition means that
    the part of the word still to be processed does not change.
    It follows that the automaton can only reach
    \[ |Q| \times {(|R| + 1)}^{|R|}\]
    configurations, which is finite.
\end{proof}



\section{Sets with atoms and orbit-finite sets}
\todo[inline]{Add seciton about sets with atoms and oribit finite sets}
\subsection{Polynomial-orbit finite sets}
Some results about sets with atoms are quite surprising. For example, they do not always admit a choice function.
\begin{example}
    Let $\binom{\atoms}{2}$ be the set of unordered pairs of atoms (i.e. sets of size two). There is no finitely supported function:
    \[f: \binom{\atoms}{2} \to \atoms\]
    such that for all $x, y$
    \[ f\left(\{x, y\}\right) \in \{x, y\}\]
\end{example}
\begin{proof}
    Suppose there is such $f$, supported by $\bar a$. Take two different atoms $x, y \not \in \bar a$ and
    and atom automorphism $\pi$ that swaps $x$ and $y$ and does not touch other atoms. This $\pi$ is clearly
    an $\bar a$-automorphism. Assume without loss of generality that $f\left(\{x, y\}\right) = x$. It follows that
    \[y = \pi(x) = \pi(f\left(\{x, y\} \right)) = f \left(\pi(\{x, y\}))\right) = f \left(\{y, x\}\right) = f\left(\{x, y\}\right) = x\]
    Which is a contraction, because $x$ and $y$ were supposed to be different.
\end{proof}
In this section we deal with those problems, following the lines of~\cite[Section B.1]{single-use-paper}
We see that (at leat part of) the problems with choice arise from the symmetry:
 \[ \{x, y\} = \{y, x\} \]
Now, we define a subclass of polynomial orbit-finite sets which does not exhibit such such symmetries.
\begin{definition}\label{def:pof}
    A \emph{polynomial orbit-finite set} is any set that can be obtained using the following grammar:
    \[ P ::= 1 \;|\; \mathbb{A} \;|\; P_1 + P_2 \;|\; P_1 \times P_2\]
    Where
    \begin{itemize}
        \item $1$ denotes the following singleton set: $\{ () \}$;
        \item $\mathbb{A}$ denotes the set of all atoms;
        \item $T_1 + T_2$ denotes the disjoint sum;
        \item and $T_1 \times T_2$ denotes the cartesian product.
    \end{itemize}
\end{definition}
As shown in \cite[Lemma~20]{single-use-paper}, polynomial orbit finite sets admit a certain kind of choice:
\begin{lemma}\label{lem:pof-uniformisation}
    Let $R \subseteq X \times Y$ be a finitely-supported relation on polynomial orbit finite sets,
    such that for every $x \in X$, its image under $R$:
    \[ x\,R = \{ y \; :\;  x \, R \, y\}\]
    is nonempty.  Then $R$ can be uniformised, i.e. there exists a finitely supported function
    \[f : X \to Y\]
    such that all $x \in X$ satisfy $x \, R \, f(x)$.
\end{lemma}
\todo[inline]{Restate the proof? Add the $\mathtt{supp}$ function, define dimension}


\section{Deterministic orbit-finite automata}
\todo[inline]{Add section about orbit-finite automata}

\section{Orbit-finite semigroups}
\todo[inline]{Add section about orbit-finite semigroups}

==> su-abstract-automata.tex <==
\section{Single-use automata}
With the help of single-use functions, we can define a more general class of automata, which recognizes
languages over all polynomial orbit-finite monoids.
\begin{definition}\label{def:abstract-su-automata}
    A \emph{single-use automaton} consists of:
    \begin{itemize}
        \item a polynomial orbit-finite alphabet $\Sigma$
        \item an \emph{input multiplication factor} $k \in \mathbb{N}$
        \item an orbit-finite set of states $Q$ with a distinguished initial state $q_0 \in Q$
        \item a single-use transition function
            \[\delta : \underbrace{Q}_{\textrm{old state}} \times \underbrace{\Sigma^k}_{\textrm{input letter copied $k$ times }} \suto
            \underbrace{Q}_{\textrm{new state}} \]
        \item a single-use acceptance function $F : Q \suto  \{\yes, \no \}$
    \end{itemize}
\end{definition}
Single-use automaton recognizes a languages over its input alphabets. Its semantics is straight-forward.
When the input alphabet is $\atoms$, then single-use automata and single-use register automata are equivalent.
\begin{lemma}\label{lem:su-register-su-abstract}
    A language $L \subseteq \atoms^*$ is recognised by a single-use register automaton iff it is recognised
    by a single-use automaton\footnote{The names of the automata are confusing, but after proving this
    lemma we will only talk about single-use automata.}
\end{lemma}
\begin{proof}
    $(\Rightarrow)$: A single-use register automaton can simulate the single-use automaton. As noted before,
    polynomial orbit finite sets are isomorphic to enumerative sets. Thanks to that
    we can remember state of the single-use automaton as a state of the register automaton:
    the label in control state and the tuple of atoms in registers. Moreover, single-use register
    automaton can compute single-use functions -- it goes along the decision tree, remembering its position
    in the control state.\\
    $(\Leftarrow)$: First, by Corollary~\ref{corollary:su-one-way-can-never-fail} we assume that
    the register automaton recognising $L$ behaves well on all inputs. Now, we need to show
    that the behaviour of one letter word can be expressed as single-use function:
    \[ f: \underbrace{Q \times {(\atoms + \bot)}^R}_{\textrm{input state}} \times
       \underbrace{\atoms^k}_{\substack{\textrm{$k$ copies of} \\
                                        \textrm{the one-letter word}}} \suto
    \underbrace{Q \times {(\atoms + \bot)}^R + \accept + \reject}_{\textrm{output state}} \]
    for some $k \in \nat$. To do that, we notice that for every $m \in \nat$, a function that
    simulates one step of the computation, is a single-use function:
    \[ f_m : \underbrace{Q \times {(\atoms + \bot)}^R}_{\textrm{input state}} \times
    \underbrace{\atoms^m}_{
        \substack{\textrm{$m$ copies of} \\
        \textrm{the input}}} \suto
 \underbrace{Q \times {(\atoms + \bot)}^R \times \atoms^{m-2}}_{\substack{
     \textrm{the automaton stayed}\\
     \textrm{in the current position;}\\
     \textrm{we remember new state}\\
     \textrm{and $m-2$ copies of the letter}
 }} + 
 \underbrace{Q \times {(\atoms + \bot)}^R + \accept + \reject}_{\substack{
    \textrm{the automaton went forward,}\\
    \textrm{accepted, or rejected}
 }} \]
Indeed, we can implement it, as a forest of trees with at most one query -- the one requested
by the automaton in a given control state. The function uses the input letter at most twice:
once for the query and once for the action. Thanks to that, it is always going to have
at least $m-2$ unused copies of the input letter to return. Now, notice that the one-letter
behaviour function can be expressed as a composition of one-step functions:
\[f = f_{2}' \circ f_4' \circ \ldots f_{2k}\]
where $k$ comes from Corollary~\ref{corollary:su-bounded}, and $f_i'$ is the function $f_i$ extended
by identity to the matching domain. It follows that $f$ is a single-use function,
as composition of single-use functions. Which means that every single-use register automaton
can be simulated by a single-use automaton, with the multiplication constant coming from Corollary~\ref{corollary:su-bounded}. 
\end{proof}
From this point on, we will no longer mention single-use register automata; single-use automata are
more convenient to use, and by Lemma~\ref{lem:su-register-su-abstract} they are also more general.\\


With this new model, the translation from automata to monoids becomes straightforward.
\begin{lemma}\label{lem:su-abstract-to-monoids}
    Each language recognized by a single-use automaton, is also recognised by a 
    orbit-finite monoid.
\end{lemma}
\begin{proof}
    The language is recognised by the monoid of behaviours: $Q \suto Q$.
    To avoid a potential confusion, it is worth pointing out, that we do not claim that either
    $(Q \suto Q) \times (Q \suto Q) \to (Q \suto Q)$,  
    or the monoid homomorphism $\Sigma^* \to Q$ are single-use functions.\\
\end{proof}

%We finish this section with a Corollary from Lemmas~\ref{lem:su-abstract-to-monoids}~and~\ref{lem:su-register-su-abstract}.
%\begin{corollary}\label{corollary:register-to-monoids}
%    Every language (over the alphabet $\atoms^*$), recognised by a single-use register automaton is also recognised
%    by an orbit-finite monoid.
%\end{corollary}

\todo[inline]{Add 2-way automata?}

==> su-automata-def.tex <==
\chapter{Single-use automata}

\section{Single-use register automata}

For the majority of this section we keep the focus on equality atoms; this way the definitions,
theorems, and proofs become clearer. In the final part, however, we
zoom out and discuss how the presented results extend to other atoms.

We start by defining single-use register automata. Its syntax is identical to the syntax of the register automaton
from Section~\ref{sec:register-automata}. Let us recall it:
\begin{definition}
    A syntax of a \emph{register automaton} consists of:
    \begin{enumerate}
        \item A finite set $Q$ of \emph{control states};
        \item An \emph{initial state} $q_0 \in Q$;
        \item A finite set $R$ of \emph{registers};
        \item A transition function which maps each control state $q \in Q$ to
        \[ \underbrace {questions}_{\textrm{what question to ask}}
         \times \underbrace{
                (Q \times actions)}_{
                    \substack{
                        \textrm{what to do if the question} \\
                        \textrm{has a ``yes'' answer}
                    }
                    }\times \underbrace{(Q \times actions)}_{\substack{
                        \textrm{what to do if the question} \\
                        \textrm{has a ``no'' answer}
                    }}\]
        with the following finite set of questions:
        \begin{enumerate}
             \item\label{q:cmp1} is the current letter equal to the value of register~$r \in R$?
             \item\label{q:cmp2} are the values of registers $r_1, r_2 \in R$ equal?
             \item has the automaton reached the end of word?
        \end{enumerate}
        and the following finite set of actions:
        \begin{enumerate}
            \item store the current letter in the register $r \in R$
            \item go forward
            \item accept / reject
            \item clear the contents of every register from $C \subseteq R$
        \end{enumerate}
    \end{enumerate}
\end{definition}
The semantics of a single-use register automaton is very similar to the syntax of a register automaton --
the only difference is that queries concerning contents of the registers (queries (a) and (b)) have
the side effect of clearing the queried registers.\\

\todo[inline]{Add examples}

Another way of thinking about single-use automata
is that they are a syntactic subset of register automata -- one in which every register query has to be followed
by an action that clears the contents of the queried registers. From this alternative definition, we immediately
conclude that Lemmas~\ref{lem:one-way-can-never-fail}~and~\ref{lem:register-bounded} work also for single-use
automata.

\begin{corollary}\label{corollary:su-one-way-can-never-fail}
    Every single-use register automaton can be modified so that, it never causes undefined behaviour.
\end{corollary}

\begin{corollary}\label{corollary:su-bounded}
    For each non-looping automaton, there is a number $k$, such that
    the automaton never stays in one position for more than $k$ steps.
\end{corollary}

Our main goal in this section is to prove that single-use automata recognize the same class of languages
as orbit-finite monoids. Let us start by showing that all languages recognized by a single-use automaton 
can also be recognized by an orbit-finite monoid. We follow the classical approach of translating
finite automata into finite monoids. Fix a single-use register automaton $\mathcal{A}$.
For every word $w \in \atoms^*$, define the behaviour of a word $w$ as a function:
\[f_w :
    \underbrace{Q \times {(\atoms + \bot)}^R}_{
        \substack{
            \textrm{the state in which }\\
            \textrm{the automaton enters } w \\
            \textrm{from the left}
        }
    }  \to
    \underbrace{Q \times {(\atoms + \bot)}^R}_{
        \substack{
            \textrm{the state in which} \\
            \textrm{the automaton leaves } w \\
            \textrm{from the right\ldots}
        }} +
    \underbrace{\accept + \reject}_{
        \substack{
            \textrm{\ldots or the information that the automaton }\\
            \textrm{has accepted or rejected its input}\\
            \textrm{while processing } w
        }
    }  \]
Notice, now that the behaviours are compositional -- behaviour $f_{uv}$ depends only on
the behaviours $f_u$ and $f_v$. In fact,
\[ f_{uv} = f_v' \circ f_u\]
if by $f_v'$ we denote $f_v$ extended by identity to the domain $Q~\times~{(\atoms~+~\bot)}^R~+~\accept~+~\reject$.
Moreover, the behaviour of a word also determines, weather $\mathcal{A}$ accepts or rejects it. Which means, that $L(\mathcal{A})$
is recognised by the monoid of all finitely-supported transformations:
\[ Q \times {(\atoms + \bot)}^R + \accept + \reject \ \to \ Q \times {(\atoms + \bot)}^R + \accept + \reject\]
The problem that remains to be solved is that this monoid is orbit-infinite. We deal with it, 
by defining \emph{single-use functions} and replacing the orbit-infinite monoid of all finitely-supported
transformations with the monoid of all single-use transformations, which turns out to be orbit finite.

\input{su-functions.tex}

\input{su-abstract-automata.tex}

\input{su-monoid-representations.tex}


==> su-monoid-representations.tex <==
\section{Single-use monoid representation}
In this section we prove the remaining inclusion:
\begin{lemma}\label{lem:monoids-to-su}
    Every language over polynomial orbit-finite alphabet
    recognised by an orbit-finite monoid, can also be recognised
    by a single-use automaton.
\end{lemma}
 For finite automata and finite monoids the construction is very easy:
the automaton keeps a monoid value in its state, and multiplies it by subsequent input letters.
When trying to apply this construction for orbit-finite semigroups and single-use automata, 
we encounter two problems. First, not all monoids have to be polynomial orbit-finite sets
(contrary to the set of states of orbit-finite), e.g.\ the syntactic monoid  of the
language over $\atoms$ ``the word contains at most 3 different atoms'':
\[ \{ X\ |\ X \subseteq \atoms,\ |X| \leq 3\} + 0 \]
A similar problem has already been studied in~\cite[Section 6.2]{bojanczyk_book}.
The other difficulty is that most of the times, the monoid multiplication function
is not single-use, e.g.\ the syntactic monoid of the language over $\atoms$,
``the word contains at most one atom'' -- the set $\atoms + 1 + 0$, with operation
defined by its $\atoms$ fragment:
\[a \cdot b =  \begin{cases}
                    a & \textrm{if $a = b$ }\\
                    0 & \textrm{otherwise}
                \end{cases}
\]
We deal with both of those problems, by considering representations of monoids compatible
with single-use functions (and polynomial orbit-finite sets):

\begin{definition}\label{def:su-representation}
    A \emph{single-use representation of a semigroup $S$} is a polynomial
    orbit-finite set $\repr{S}$, with a surjective, partial representation function: $r : \repr{S} \pto S$
    and a with single-use multiplication function: $\ast : \repr{S} \times \repr{S} \suto \repr{S}$, such that
    for all $a, b \in \repr{S}$ for which $r(a)$ and $r(b)$ are defined
    \[ r(a \ast b) =  r(a)\,r(b)  \]
\end{definition}

Note, that the function $r$ does not have to be injective, and therefore each element of $S$
may have more than one representation. Moreover, $\repr{S}$ and $\ast$
\todo{investigate wheather every language recognised by an o-f monoid, can also be recognised by a p-o-f monoid}
may not form a monoid
elements $(a \ast b) \ast c$ and $a \ast (b \ast c)$ may be different representations of the
same element.\\

\todo[inline]{Add an example?}

The core of this section is the following lemma:
\begin{lemma}\label{lem:has-su-representation}
    Every orbit-finite monoid has a single-use representation.
\end{lemma}
Before proving the lemma, we use it to translate monoids into single-use automata
(Lemma~\ref{lem:monoids-to-su}). For that, we are going to need two more technical lemmas. The first
one states that every function can be made single-use, if it gets enough copies of the argument:

\begin{lemma}\label{lem:fs-to-su}
    For every finitely supported (not necessarily single use) function between two
    polynomial orbit finite sets
    \[f : A \to B \]
    there exists a number $k$, and a single-use function $f' : A^k \suto B$, such that for every $a \in A$:
    \[f(a) = f'(\underbrace{a, a, \ldots, a}_{k \textrm{ times}})\]
\end{lemma}
\begin{proof}
    Take any finitely supported $f : A \to B$, and denote its support by $\bar{c}$.
    By definition of finitely supported function, the $\bar{c}$-orbit of
    $(a, f(a))$ is determined by the $\bar{c}$-orbit of $a$. This means that
    if we know the $\bar{c}$-orbit of the input, we know which atoms
    from $\textrm{supp}(a)$ and from $\bar{c}$, should be copied to which positions
    of the output. We can compute the $\bar{c}$-orbit of the argument,
    using $\dim(A) + |\bar{c}|$ copies of the input -- for every two atoms
    atoms from $\supp(a)$ or from $\bar{c}$, we ask if they are equal. Additionally,
    we might need up to $\dim(B)$ copies of each atom from $\supp{a}$ ore from $\bar{x}$,
    to use it in the output. This means that $f(a)$ can be computed in a single-use way,
    using
    \[k := \dim{A} + \dim{B} + |\bar{c}|\]
    copies of the input in total.    
\end{proof}

Now a useful Corollary of Lemma~\ref{lem:fs-to-su}:
\begin{corollary}\label{cor:accept-mult-use}
    The relaxed version of single-use automata where acceptance functions do not have to be
    single use (but still have to be finitely supported) has the same expressive power as
    the standard single-use automata.
\end{corollary}
\begin{proof}
    Thanks to Lemma~\ref{lem:fs-to-su} the acceptance function can be made single use,
    provided that we keep enough copies of the automaton's state. This can be done at the
    cost of increasing the input multiplication factor -- we start with enough copies of the initial state and
    than update each copy independently using the original transition function.
\end{proof}

When constructing the automaton in the proof of Lemma~\ref{lem:monoids-to-su}, we are going
to use uniformisation (from Lemma~\ref{lem:pof-uniformisation}), which has the side effect
adding arbitrary atoms to the construction. We can get rid of those, thanks to the following lemma:
\begin{lemma}\label{lem:remove-redundant}
    If a language $L$ supported by $\bar a$ is recognised by any single-use automaton,
    than it is also recognised by a single-use automaton supported by $\bar a$.
\end{lemma}
\todo[inline]{Add a proof.}

Now, assuming that Lemma~\ref{lem:has-su-representation} is correct, we prove Lemma~\ref{lem:monoids-to-su}:
\begin{proof}
    Take any language over a polynomial orbit-finite alphabet $\Sigma$ that is recognised by
    an orbit-finite monoid $M$. Let $\repr{M}$, $r$, $\ast$ be the single-use representation of $M$. Now, the construction is mostly straightforward:\\

    The initial element is a representation of monoid's neutral element.\\

    The transition function multiplies automaton's state by the element corresponding to the next letter.
    It is constructed in the following way: Take the the language's morphism function
    $m : \Sigma \to M$. Define relation $R \; \subseteq \; \Sigma \times \repr{S}$
    \[ x \, R \, y \iff m(x) = r(y) \]
    and unformise $R$ using Lemma~\ref{lem:pof-uniformisation} obtaining function
    $\repr{m} : \Sigma \to \repr{M}$ -- the lemma is applicable, because $r$ is surjective.
    Finally apply Lemma~\ref{lem:fs-to-su} to $\repr{m}$, obtaining:
   \[ \repr{m}' : \Sigma^k \suto \repr{M}\]
    Define automaton's transition function as a composition:
    \[\repr{M} \times \Sigma^{k}
    \overset{\substack{
        \textrm{apply $\repr{m}$}\\
        \textrm{to $\Sigma^{k}$}
    }}{\longsuto}
    \repr{M} \times \repr{M}
    \overset{\substack{
       (\ast)
    }}{\longsuto} \repr{M} \]

    The acceptance function is natural: first maps an element of $\repr{M}$ to an element of $M$
    (using $r$) and then checks if the element is accepting (using monoid's acceptance function).
    Thanks to Corollary~\ref{cor:accept-mult-use}, we do not have to worry if this function is single-use.\\

    We finish the construction by noting that the multiplication factor of the automaton is $k$.
\end{proof}

We are now left with proving Lemma~\ref{lem:has-su-representation}. Before the proof, we look at
Green's relations, presented according~to~\cite[Section V.1]{pin2010mathematical}.

\begin{definition}\label{def:green-order}
    Let $S$ be a semigroup, we define three preorders on its elements:
    \begin{itemize}
        \item $s \emph{\prefix} t$ if there exists $u \in S$ such that $su = t$, or $s = t$
        \item $s \emph{\sufix} t$ if there exists $u \in S$ such that $us = t$, or $s = t$
        \item $s \emph{\infix} t$ if there exists $u, v \in S$ such that $usv = t$, or $s = t$
    \end{itemize}
    and four equivalence relations:
    \begin{itemize}
        \item $s \emph{\prefequiv} t$ if $s \prefix t$ and $t \prefix s$
        \item $s \emph{\sufequiv} t$ if $s \sufix t$ and $t \sufix s$
        \item $s \textrm{\emph{ is }} \Jj \textrm{\emph{- (infix-) equivalent to t}}$ ($s \infequiv t$) if $t \infix s$ and $s \infix t$ 
        \item $s \textrm{\emph{ is }} \mathcal{H}\textrm{\emph{-equivalent with t}}$ ($s \hequiv t$) if $s \prefix t$ and $s \sufix t$ 
    \end{itemize}
\end{definition}

Those relations are used to define $\Jj$-height -- a parameter measuring the potential of each element to develop
in the $\Jj$-hierarchy:
\begin{definition}\label{def:j-height}
    Let $S$ be a semigroup. Define \emph{$\Jj$-height} of an element from $S$, to be
    the maximal length of a $\Jj$-chain starting in that element. A $\Jj$-chain
    is a sequence of elements $x_1, \ldots, x_k \in S$, such that
    $x_{i} \infix x_{i+1}$, but $x_{i+1} \textrm{ is not an infix of } x_i$.
    A $\Jj$-height of a monoid is the maximal $\Jj$-height of its element.
\end{definition}

It turns out that if we work with equality atoms, the $\Jj$ height has to be limited.
\begin{lemma}
    For equality atoms, the $\Jj$-height of every orbit-finite semigroup is finite.
\end{lemma}
\begin{proof}
    Let $S$ be an orbit-finite semigroup, supported by $\bar a$.
    \begin{claim}
        If elements $x, y \in S$ are in the same $\bar a$-orbit, then they are either $\Jj$-equivalent
        or $\Jj$-incomparable.
    \end{claim}
    \begin{proof}
       It suffices to show, that for every $x \in S$ and for every $\bar{a}$-automorphism $\pi$:
       if $x \prefix \pi(x)$, $\pi(x) \prefix x$. Since we are working with equality
       atoms, we can assume without loss of generality that $\pi$ only touches finitely-many atoms. It follows that
       there is a number $k$, such that $\pi^k$ is the identity function. Every support of the monoid also
       supports the prefix relation (because it depends equivariantly on the monoid). This means that
       \[\pi(x) \prefix \pi(\pi(x))\]
       which in turn means that 
       \[\pi^2(x) \prefix \pi^3(x)\] 
       and so on\ldots.
       By repeating the process we finally obtain that
       \[\pi^{k-1}(x) \prefix \pi^k(x) = x\]
       which closes the cycle and shows that all $x_1, \ldots x_k$ are  $\Jj$-equivalent to each other.
    \end{proof}
    Thanks to the Claim, we see that no $\Jj$-chain contains two elements from the same orbit.
    Therefore the length of every $\Jj$-chain is limited by the number of orbits in $S$.
\end{proof}

